RMQFMU: Bridging the Real World with Co-simulation Technical Report

In this paper we present an experience report for the RMQFMU, a plug and play tool, that enables feeding data to/from an FMI2-based co-simulation environment based on the AMQP protocol. Bridging the co-simulation to an external environment allows on one side to feed historical data to the co-simulation, serving different purposes, such as visualisation and/or data analysis. On the other side, such a tool facilitates the realisation of the digital twin concept by coupling co-simulation and hardware/robots close to real-time. In the paper we present limitations of the initial version of the RMQFMU with respect to the capability of bridging co-simulation with the real world. To provide the desired functionality of the tool, we present in a step-by-step fashion how these limitations, and subsequent limitations, are alleviated. We perform various experiments in order to give reason to the modifications carried out. Finally, we report on two case-studies where we have adopted the RMQFMU, and provide guidelines meant to aid practitioners in its use.

==> Diagrams/rbmq-seq-diag_DOSTEP.tex <==

\tikzumlset{font=\footnotesize}
\begin{tikzpicture}
\begin{umlseqdiag}
\umlboundary[no ddots]{Co-simulation Master}
\umlobject[no ddots]{rbmqFMUinterface}
\umlobject[no ddots]{rbmqFMUcore}
\umldatabase[no ddots, fill=yellow!20]{RabbitMQ Server}

\begin{umlcall}[op={doStep(time,stepSize)}, dt=10, padding=.5]{Co-simulation Master}{rbmqFMUinterface} \end{umlcall}

\begin{umlcallself}[op={simTime=applyPrecision(time,stepSize)}, padding=1]{rbmqFMUinterface} \end{umlcallself}
\begin{umlcall}[op={publishSHD(time) on CSHD}, dt=5, padding=.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlcall}[op={process(simTime)}, dt=5, padding=.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}


\begin{umlfragment}[type=process function] 
\begin{umlcallself}[op={check()},dt=5, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcallself}[op={processIncoming()}, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcallself}[op={processLookahead()}, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcallself}[op={processResult$=$check()}, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcall}[type=return, op={initializeResult}, dt=56, padding=0.5] {RabbitMQ Server}{rbmqFMUinterface}\end{umlcall}
\end{umlfragment}

\begin{umlcallself}[op={startTime = Time Now}, padding=1, dt=6] {rbmqFMUinterface}\end{umlcallself}

\begin{umlfragment}[type=loop,
label=TimeNow $-$ StartTime $<$ TimeOut, inner ysep=1]
\begin{umlcall}[op={consumeSingleMessage(\&msg) on CCD}, dt=6, padding=0.5]{rbmqFMUinterface}{RabbitMQ Server} \end{umlcall}

\begin{umlfragment}[type=alt ,
label=There is a msg,
inner xsep=1, inner ysep=.1] 
\begin{umlcall}[type=return,op={msg $=$ message: return True},dt=6, padding=0.5] {RabbitMQ Server}{rbmqFMUinterface} \end{umlcall}

\begin{umlcall}[op={AddToIncomUnproc(msg)}, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlfragment}[type=alt ,
label=There is change of inputs,
inner xsep=1, inner ysep=5] 
\begin{umlcall}[op={toJson(\&outgoingMsg)}, dt=12, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}
\begin{umlcall}[op={publish(outgoingMsg) on CCD},dt=5, padding=0.5]{rbmqFMUinterface} {RabbitMQ Server} \end{umlcall}
\end{umlfragment}

\begin{umlcall}[op={checkSHD(\&rT\_rec, \&sT\_rec)},dt=10, padding=0.5]{rbmqFMUinterface} {rbmqFMUcore} \end{umlcall}

\begin{umlcall}[op={processResult$=$process()}, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlfragment}[type=alt ,
label=There is valid SHD,
inner xsep=1, inner ysep=5] 
\begin{umlcall}[op={calcTimeDiff(rT\_rec, sT\_rec)}, dt=12, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlcall}[op={calcTimeDiff(time, sT\_rec)}, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}
\end{umlfragment}

\begin{umlfragment}[type=alt ,
label=ProcessResult is True,
inner xsep=1, inner ysep=5] 
\begin{umlcall}[type=return, op={True}, dt=16, padding=0.5]{rbmqFMUinterface} {Co-simulation Master} \end{umlcall}
\end{umlfragment}

\umlfpart[No msgs] \begin{umlcall}[type=return, op={False}, dt=50,padding=0.5] {RabbitMQ Server}{rbmqFMUinterface} \end{umlcall}
\end{umlfragment}

\end{umlfragment}

\begin{umlcall}[type=return, op={False}, dt=-9,padding=0.5] {rbmqFMUinterface}{Co-simulation Master} \end{umlcall}
\end{umlseqdiag}
\end{tikzpicture}


==> Diagrams/rbmq-seq-diag_ENTERINITMODE.tex <==

\tikzumlset{font=\footnotesize}
\begin{tikzpicture}
\begin{umlseqdiag}
\umlboundary[no ddots]{Co-simulation Master}
\umlobject[no ddots]{rbmqFMUinterface}
\umlobject[no ddots]{rbmqFMUcore}
\umldatabase[no ddots, fill=yellow!20]{RabbitMQ Server}

\begin{umlcall}[op={EnterInitMode}, dt=10, padding=.5]{Co-simulation Master}{rbmqFMUinterface} \end{umlcall}

\begin{umlcallself}[op={configure() CCD}, padding=1]{rbmqFMUinterface} \end{umlcallself}

\begin{umlcall}[op={Publish 'Ready Msg' on CCD}, dt=10, padding=.5]{Co-simulation Master}{RabbitMQ Server} \end{umlcall}

\begin{umlcallself}[op={configure() CSHD}, dt=7, padding=1]{rbmqFMUinterface} \end{umlcallself}

\begin{umlcallself}[op={initCoreState()}, padding=1]{rbmqFMUinterface} \end{umlcallself}

\begin{umlcallself}[op={set StartTime = TimeNow}, padding=1]{rbmqFMUinterface} \end{umlcallself}

\begin{umlfragment}[type=loop,
label=TimeNow $-$ StartTime $<$ TimeOut, inner ysep=1]
\begin{umlcall}[op={ConsumeSingleMessage on CCD}, dt=6, padding=0.5]{rbmqFMUinterface}{RabbitMQ Server} \end{umlcall}

\begin{umlfragment}[type=alt ,
label=There is a msg,
inner xsep=1, inner ysep=.1] 
\begin{umlcall}[type=return,op={msg $=$ message: return True},dt=6, padding=0.5] {RabbitMQ Server}{rbmqFMUinterface} \end{umlcall}

\begin{umlcall}[op={AddToIncomUnproc(msg)}, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlcall}[op={initializeResult$=$initialize()}, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}


\begin{umlfragment}[type=initialize function] 
\begin{umlcallself}[op={processIncoming()},dt=5, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcallself}[op={processLookahead()}, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcallself}[op={calculateStartTime()}, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcallself}[op={initializeResult$=$check(0)}, padding=1] {rbmqFMUcore}\end{umlcallself}

\begin{umlcall}[type=return, op={initializeResult}, dt=35, padding=0.5] {RabbitMQ Server}{rbmqFMUinterface}\end{umlcall}
\end{umlfragment}


\begin{umlfragment}[type=alt ,
label=InitResult is True,
inner xsep=1, inner ysep=5] 
\begin{umlcall}[type=return, op={True}, dt=12, padding=0.5]{rbmqFMUinterface} {Co-simulation Master} \end{umlcall}
\end{umlfragment}

\umlfpart[No msgs] \begin{umlcall}[type=return, op={False}, dt=13,padding=0.5] {RabbitMQ Server}{rbmqFMUinterface} \end{umlcall}
\end{umlfragment}

\end{umlfragment}

\end{umlseqdiag}
\end{tikzpicture}


==> Diagrams/rbmq-seq_CHECKSHD.tex <==

\tikzumlset{font=\footnotesize}
\begin{tikzpicture}
\begin{umlseqdiag}
\umlobject[no ddots]{rbmqFMUinterface}
\umlobject[no ddots]{rbmqFMUcore}
\umldatabase[no ddots, fill=yellow!20]{RabbitMQ Server}

\begin{umlcallself}[op={tryAgain=true},dt=10, padding=0.9]{rbmqFMUinterface}  \end{umlcallself}

\begin{umlfragment}[type=loop,
label={tryAgain}, inner ysep=1]

\begin{umlcall}[op={consumeSingleMessage(\&msgSH) on CSHD}, dt=6, padding=0.5]{rbmqFMUinterface}{RabbitMQ Server} \end{umlcall}

\begin{umlfragment}[type=alt ,
label=There is a message,
inner xsep=1, inner ysep=5] 

\begin{umlcall}[op={\parbox[c]{2.5cm}{\centering valid$=$parseMsg(\&rT, \&sT,msgSH)}}, dt=14, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlfragment}[type=alt ,
label=valid=True,
inner xsep=1, inner ysep=5] 

\begin{umlcall}[op={{\centering rt$=$toSimTime(rT\_received)}}, dt=12, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}

\begin{umlcall}[op={{\centering st$=$toSimTime(sT\_received)}}, padding=0.5]{rbmqFMUinterface}{rbmqFMUcore} \end{umlcall}


\end{umlfragment}

\umlfpart[No msg] \begin{umlcallself}[op={tryAgain=false}, padding=0.9]{rbmqFMUinterface}  \end{umlcallself}
\end{umlfragment}


\end{umlfragment}

\end{umlseqdiag}
\end{tikzpicture}


==> Figures/rbmqv1/urdata/timegaps.tex <==
\begin{tikzpicture}
    \pgfplotstableread[col sep=comma]{raw_data/rbmqv1/urdata/ur_timegaps_short.csv}\datatable
    \pgfplotstablegetrowsof{\datatable}
    \pgfmathsetmacro{\N}{\pgfplotsretval} 
    \begin{axis}[ylabel={Data time gap ($ms$)}, 
                    xlabel={Data time offset ($ms$)},
                    height=6cm,width=8cm,
                    title={Time gaps in the data},
                    clip=false,
                    %xmajorgrids=true,
                    %ymajorgrids=true,
                    scaled x ticks=base 10:-3,
             ]   

            \addplot[mark=none, cyan] table[x index = {3},y index = {2},skip coords between index={700}{\N}] \datatable;
    \end{axis}
\end{tikzpicture}

==> Listings/msg2Consume_SHD.tex <==
\begin{lstlisting}[language=json,firstnumber=1]
{
    "rtime":"2019-01-04T16:41:24+02:00",
    "cosimtime":"2019-01-04T16:41:24+02:00",
}
\end{lstlisting}

==> Listings/msg2Send_SHD.tex <==
\begin{lstlisting}[language=json,firstnumber=1]
{
    "simAtTime":"2019-01-04T16:41:24+02:00"
}

\end{lstlisting}

==> Tables/experiments_table_cas2.tex <==
\begin{table}[]
\centering
\caption{Overview of experiments for Case-study 2}
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{\textbf{Case-study 1}} & \multicolumn{5}{c}{Parameters}                         \\

                                       & lA & mA & $t_s$ & $f_{data}$ & threaded     \\
                                       \midrule
Case 1                                 & 1         & 0.2s   & 0.1s      & every 0.1s & yes      \\
\midrule
Case 2                                 & 50         & 0.2s     & 0.1s       & every 0.1s & yes      \\
\midrule
Case 3                                 & 1         & 2s   & 0.1s      & every 0.1s & yes      \\
\midrule
Case 4                                 & 50         & 2s     & 0.1s       & every 0.1s & yes      \\
\midrule
Case 5                                 & 50         & 0.2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 6                                 & 200         & 2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 7                                 & 50         & 0.2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 8                                & 200         & 2s     & 0.1s       & every 0.002s & yes      \\
\midrule
Case 9                                & 2         & 0.4s     & 0.1s       & every 0.2s & yes      \\
\midrule
Case 10                                & 5         & 0.4s     & 0.1s       & every 0.2s & yes      \\
\midrule
Case 11                                 & 2         & 2s     & 0.1s       & every 0.2s & yes      \\
\midrule
Case 12                                & 5         & 2s     & 0.1s       & every 0.2s & yes      \\



\bottomrule
\end{tabular}
\end{table}

==> rbmqFMU_currentDesign.tex <==
\section*{RabbitMQ current design - Not part of the paper structure}
\begin{figure}
    \centering
    \resizebox{\textwidth}{!}{
    \input{Diagrams/rbmq-seq-diag_ENTERINITMODE}
    }
    \caption{Sequence Diagram for the function: $EnterInitializationMode$}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.9\textwidth}{!}{
    \input{Diagrams/rbmq-seq-diag_DOSTEP}
    }
    \caption{Sequence Diagram for the function: $DoStep$}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.9\textwidth}{!}{
    \input{Diagrams/rbmq-seq_CHECKSHD}
    }
    \caption{Sequence Diagram for the function: $checkSHD$, that deals with consumed system health data.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.6\textwidth}{!}{
    \input{Listings/msg2Send_SHD}
    }
    \caption{Message on system health data published by the rabbitMQFMU.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \resizebox{.6\textwidth}{!}{
    \input{Listings/msg2Consume_SHD}
    }
    \caption{Message on system health data consumed by the rabbitMQFMU}
    \label{fig:my_label}
\end{figure}
